Optimal Decision Lists using SAT

Decision lists are one of the most easily explainable machine learning models. Given the renewed emphasis on explainable machine learning decisions, this machine learning model is increasingly attractive, combining small size and clear explainability. In this paper, we show for the first time how to construct optimal "perfect" decision lists which are perfectly accurate on the training data, and minimal in size, making use of modern SAT solving technology. We also give a new method for determining optimal sparse decision lists, which trade off size and accuracy. We contrast the size and test accuracy of optimal decisions lists versus optimal decision sets, as well as other state-of-the-art methods for determining optimal decision lists. We also examine the size of average explanations generated by decision sets and decision lists.

==> maxsat.tex <==
\subsection{MaxSAT Model} \label{sec:maxsat}

\begin{comment}
Rather than using the described iterative SAT-based procedure, which
iterates over varying size $N$ of the target decision set, we can
allocate a predefined number of nodes, which serves as an upper bound
on the optimal solution, and formulate a MaxSAT problem minimizing the
number of nodes used.
%
\end{comment}
Let us add a flag variable $u_j$ for every available node.
%
Variable $u_j$ is \emph{true} whenever the node $j$ is unused and
\emph{false} otherwise.
%
% The MaxSAT model is as follows:
Consider the following constraints:
%
\begin{enumerate}
%
\item A node either decides a feature or is unused:
%
\begin{equation}\label{eq:used} \forall_{j \in [N]}\ u_j +
\sum_{r\in[K+1]} s_{jr} = 1 \end{equation}
%
\ignore{ \item A node $j$ assigns a value to feature $f_r$, i.e.\
  %
  $$
  %
  \begin{array}{cl}
      %
      \forall_{j\in[N]} \forall_{r\in[K+1]}\ a_{jr}^0\leftrightarrow &
      (s_{jr} \land \neg{t_j}) \\
      %
      \forall_{j\in[N]} \forall_{r\in[K+1]}\ a_{jr}^1\leftrightarrow &
      (s_{jr} \land t_j) \\
      %
  \end{array}
  %
  $$ }
%
\item If a node $j$ is unused then so are all the following nodes
%
\begin{equation}\label{eq:newlast} \forall_{j \in [N-1]}\ u_{j}
\rightarrow u_{j+1} \end{equation}
%
\item The last used node is a leaf
%
\begin{eqnarray}
\forall_{j \in [N-1]}\ u_{j+1} \rightarrow u_j \vee s_{jc} \\
u_{N} \vee s_{Nc}
\end{eqnarray}
%
\ignore{
\item All examples are valid at the first node
%
$$\forall_{i \in [M]}\ v_{i1}$$
%
\item An example $e_i$ is valid at node $j+1$ iff $j$ is a leaf
  node, or $e_i$ is valid at node $j$ and $e_i$ and node $j$ agree
  on the value of the feature $s_{jr}$ selected for that node:
  %
  % $$\forall_{i \in [M]} \forall_{j \in [N-1]}\ v_{ij+1}
  % \leftrightarrow s_{jc} \vee (v_{ij} \wedge \bigvee_{r\in[K]}
  % (s_{jr} \wedge (\pi_{i}[r] = t_j)) $$
  %
  $$
  %
  \forall_{i \in [M]} \forall_{j \in [N-1]}\ v_{ij+1}
  \leftrightarrow s_{jc} \vee (v_{ij} \wedge \bigvee_{r\in[K]}
  {a_{jr}^{\pi_i[r]}})
  %
  $$
%
\item If example $e_i$ is valid at a leaf node $j$, they should
  agree on the class feature, i.e.\
  %
  %$$
  %%
  %\forall_{i \in [M]} \forall_{j \in [N]}\ (s_{jc} \wedge v_{ij})
  %\rightarrow (c_i = t_j)
  %%
  %$$
  $$
  %
  \forall_{i \in [M]} \forall_{j \in [N]}\ (s_{jc} \wedge v_{ij})
  \rightarrow a_{jc}^{\pi_i[c]}
  %
  $$
%
\item For every example there should be at least one leaf literal
  where it is valid: $$\forall_{i \in [M]}\
  \bigvee_{j\in[N]}(s_{jc} \wedge v_{ij})$$
%
}
\end{enumerate}

The constraints above together with
constraints~\noas{\eqref{eq:assign}, }\eqref{eq:vfirst},\eqref{eq:nfirst}, \eqref{eq:valid}, \eqref{eq:nassign},\eqref{eq:class}, and \eqref{eq:correct} comprise
the hard part of the MaxSAT formula, i.e.\ every clause of it must be
satisfied.
%
As for the optimization criterion, we maximize $\sum_{j \in [N]} u_j$,
which can be trivially represented as a list of unit soft clauses of
the form $(u_j, 1)$.

\begin{comment}
The model is still used iteratively in the worst case. We guess an upper bound $N$ on the size of the decision set.
We use the model to search for a decision set of size less than or equal to $N$.  If this fails we increase $N$ by some number
(say 10) and retry, until the time limit is reached.


\begin{example}
Revisiting the solution shown in \autoref{ex:data} when $N$ is set to 9
we find the solution illustrated in \autoref{ex:soln}
extended so that the last two nodes are unused: $u_8 = u_9 = \true$.
The last used node 7 is clearly a leaf. Note that validity ($v_{ij}$) and truth
value ($t_j$) variables are irrelevant to unused nodes $j$.
\ignore{
The critical decisions are given in
the following table.
$$
\begin{array}{l|ccccccccc}
& 1 & 2 & 3 & 4 & 5 & 6 & 7 & 8 & 9 \\ \hline
s_{jr},u_j & s_{1L} & s_{2H} & s_{3L} & s_{4C} & s_{5H} & s_{6C} & s_{7H} &
u_{8} & u_9 \\
t_{j}  & \true  & \false  & \false & \false & \true   & \true  & \false  & \mbox{---} &
\mbox{---} \\
v_{ij} & v_{11}  & v_{12} & v_{13} & v_{34} & v_{35} & v_{16} & v_{47} &
v_{18} & \\
       & \vdots & v_{22} & \vdots & v_{54}  &  v_{55} & \vdots  & v_{67} &
\vdots & \\
       &  v_{81} &  v_{42}  & v_{83} &  v_{74} &  v_{85} &  v_{86} &  v_{77}
& v_{88} & \\
       &  &  v_{62} &  & v_{84} &  &  & & & \\
\end{array}
$$
Note the truth value $t_j$ and validity $v_{ij}$ is irrelevant in unused
nodes $j$, and the last used node 7 is a leaf.
}
\qed
\end{example}
\end{comment}

